AlignRec: Aligning and Training in Multimodal Recommendations

With the development of multimedia systems, multimodal recommendations are playing an essential role, as they can leverage rich contexts beyond interactions. Existing methods mainly regard multimodal information as an auxiliary, using them to help learn ID features; However, there exist semantic gaps among multimodal content features and ID-based features, for which directly using multimodal information as an auxiliary would lead to misalignment in representations of users and items. In this paper, we first systematically investigate the misalignment issue in multimodal recommendations, and propose a solution named AlignRec. In AlignRec, the recommendation objective is decomposed into three alignments, namely alignment within contents, alignment between content and categorical ID, and alignment between users and items. Each alignment is characterized by a specific objective function and is integrated into our multimodal recommendation framework. To effectively train AlignRec, we propose starting from pre-training the first alignment to obtain unified multimodal features and subsequently training the following two alignments together with these features as input. As it is essential to analyze whether each multimodal feature helps in training and accelerate the iteration cycle of recommendation models, we design three new classes of metrics to evaluate intermediate performance. Our extensive experiments on three real-world datasets consistently verify the superiority of AlignRec compared to nine baselines. We also find that the multimodal features generated by AlignRec are better than currently used ones, which are to be open-sourced in our repository https://github.com/sjtulyf123/AlignRec_CIKM24.

==> expired/methods-old.tex <==
\section{Proposed Framework}
\subsection{Framework Overview}
The overview of our proposed framework, Align4Rec, is illustrated in Fig.~\ref{fig:framework}. As discussed before, the whole framework consists of three alignment stages with an intermediate evaluation module. In this section, we will first introduce the alignment stages, and then show our detailed designs of network structures. The training strategies with intermediate evaluation protocols will be discussed in Sec.~\ref{sec:train}.

\subsection{Three-stage Alignment}
In this part, we will introduce the motivations and designs of our three alignment stages. As discussed before, many studies in multimodal large models~\cite{li2021align,lin2023vila} explore the necessity of aligning image and text features and the following gains in cross-modality understanding. Regarding ID as special categorical modalities motivates us to analyze the alignment issue in multimodal recommendation and propose the Align4Rec.
Generally, our framework contains the input of user's ID $u_{id}$, interacted item's ID $i_{id}$, item's raw images $i_v$, and item's raw text $i_t$. The goal of three-stage alignment is to generate an aligned items and users representations $\mathbf{h}_{i}$ and $\mathbf{h}_u$ containing rich multimodal knowledge for the final top-K recommendation.

\subsubsection{Inter-Modality Alignment}
In multimodal recommendation scenarios, item's vision modality and text modality usually illustrate the same item from different aspects (\eg, pictures and descriptions of the same product). However, extracting vision and text features from different encoders will result in the distribution and representation gap between modalities, making it hard for item representations. In Fig.~\ref{fig:motivations}(a), we show the t-SNE~\cite{van2008visualizing} results of vision and text features which are commonly used in multimodal recommendation in Amazon Sports dataset~\cite{he2016ups}. We find that have very different distributions so vision-text pairs can be far apart, since they are extracted from VGG and Transformer, separately.

Therefore, inspired by the advanced image-text pre-training schema, we propose to adopt a transformer-based multimodal encoder to generate a unified multimodal representation by aligning vision and text information. Formally, suppose $MMEnc$ is a general multimodal encoder, and $h_{enc}^i$ is the unified representation for item $i$'s vision and text, then the inter-modality alignment stage is:
\begin{align}\label{eq:mmrec}
    \textbf{h}_{enc}^i = MMEnc(i_v,i_t)\,.
\end{align}

In Eq.~\eqref{eq:mmrec}, the vision-text alignment is optimized through the cross-attention based transformers in $MMEnc$. In implementations, we utilize the most advanced BEiT3~\cite{wang2022image} as the backbone and adopt its' mask-data-modeling techniques to mask some tokens of one modality (\eg, vision) while predicting the masked token using another modality (text) and remaining tokens in the masked modality (vision). In this way, the $MMEnc$ can attend to both vision and text information so that the multimodal information is gradually aligned and fused. The training loss of this stage can be written as the sum of mask-image-modeling (MIM) and mask-language-modeling (MLM) in Eq.~\eqref{eq:mmrec-loss}. After that, we obtain the \textbf{CLS} token as the unified multimodal representation $\textbf{h}_{mm}^i$.
\begin{align}\label{eq:mmrec-loss}
    \mathcal{L}_{IMA} = \mathcal{L}_{MIM}+\mathcal{L}_{MLM}\,.
\end{align}

\subsubsection{Modality-ID Alignment}
After obtaining a unified encoded multimodal representation $\mathbf{h}^i_{enc}$ for each item, we try to aggregate items' and users' multimodal and ID-based information based on the user-item interacted graph $\mathcal{G}$. However, as presented in Fig.~\ref{fig:motivations}(b), the t-SNE results of the same item's multimodal and item ID feature without alignment can be far away. It indicates that simply adopting aggregating layers (\eg, MLP or GCN) to acquire multimodal and ID high-level hidden representations separately will make the distance within the same modality-ID pair far. In this case, the model is hard to distinguish between modality-ID pairs of different items and users. Therefore, we try to do alignment between multimodal and ID hidden representations of the same user or item in this stage after aggregation. Generally, suppose $Aggregator$ is an aggregation module which can be GCN or other neural networks. It will output user/item multimodal hidden representations ($\mathbf{h}^u_{mm}$, $\mathbf{h}^i_{mm}$) and ID-based representations ($\mathbf{h}^u_{id}$, $\mathbf{h}^i_{id}$)) with the help of the interaction graph $\mathcal{G}$:
\begin{align}\label{eq:aggregation}
    \mathbf{h}^i_{mm}, \mathbf{h}^u_{mm}, \mathbf{h}^i_{id}, \mathbf{h}^u_{id}=Aggregator(\mathbf{h}^i_{enc},i_{id},u_{id}|\mathcal{G})\,.
\end{align}

After that, we utilize the in-batch InfoNCE~\cite{zhao2023augmented,he2020momentum} to model the modality-ID alignment, guiding our framework learning the difference of positive and negative modality-ID pairs. Denote $i'$ and $u'$ as in-batch items and users, separately; Denote $\tau$ as the temperature hyper-parameter. Then the modality-ID alignment task can be optimized through:
\begin{align}\label{eq:agg-loss}
    \mathcal{L}_{MIA}=-\log \frac{\exp (\mathbf{h}^i_{mm}\cdot \mathbf{h}^i_{id}/\tau)}{\sum_{i'} \exp (\mathbf{h}^i_{mm}\cdot \mathbf{h}^{i'}_{id}/\tau)}-\log \frac{\exp (\mathbf{h}^u_{mm}\cdot \mathbf{h}^u_{id}/\tau)}{\sum_{u'} \exp (\mathbf{h}^u_{mm}\cdot \mathbf{h}^{u'}_{id}/\tau)}\,.
\end{align}

Aside from the alignment task, the multimodal hidden representation itself also contains rich information: Similar items' multimodal information should also be similar. It can help our framework build the relationship among items. Besides, the multimodal hidden representation $\mathbf{h}^i_{mm}$ will be blindly optimized towards the ID representation $\mathbf{h}^i_{id}$ during the modality-ID alignment stage, leading to a representation collapse~\cite{javaloy2022mitigating} problem and losing its semantic information. Therefore, to keep the similarity relationship among multimodal features and avoid representation collapse, we propose an in-batch regularizer to constrain the similarity between each two multimodal hidden representation $\mathbf{h}^i_{mm}$ stay close to the similarity between $\mathbf{h}^i_{enc}$. Denote $i$ and $j$ are two in-batch items, $C(\mathbf{x},\mathbf{y})$ as the cosine similarity between two vectors, $||\cdot||_2$ as the L2-norm, $sg(\cdot)$ as the stop gradient operator; Then the regularizer can be defined as follows:

\begin{align}\label{eq:sim-loss}
    \mathcal{L}_{reg} = ||C(\mathbf{h}^i_{mm},\mathbf{h}^j_{mm})-sg( C(\mathbf{h}^i_{enc},\mathbf{h}^j_{enc}))||_{2}\,.
\end{align}

\subsubsection{User-Item Alignment}
The multimodal hidden representations and ID-based representations contain the information of item/user from different fields or aspects. In our Aign4Rec framework, we first use a fusion module $Fuser$ to fuse these information into general item/user representations $\mathbf{h}^i$ and $\mathbf{h}^u$ in Eq~\eqref{eq:fusion}, and then try to align the representation space between users and their interacted items. We conduct this user-item alignment because we intend to maximize the prediction of the interacted item $i$ given a user $u$, which will help learn the recommendation goal in Eq.~\eqref{defi:bpr}.
\begin{align}\label{eq:fusion}
    \mathbf{h}^i=Fuser(\mathbf{h}^i_{mm}, \mathbf{h}^i_{id}),\quad \mathbf{h}^u=Fuser(\mathbf{h}^u_{mm}, \mathbf{h}^u_{id})\,.
\end{align}

Afterwards, we build the user-item alignment task with a cosine similarity loss between the user final representation $\mathbf{h}^u$ and corresponding interacted item $\mathbf{h}^i$:
\begin{align}\label{eq:ui-loss}
    \mathcal{L}_{UIA}=1-C(\mathbf{h}^i,\mathbf{h}^u)\,.
\end{align}

\subsection{Detailed Structure Design}
Our Align4Rec framework mainly focuses on the alignment design and simplifies the concrete network structure into three necessary modules, which enhances the generalizability of our framework. Specifically, the multimodal encoder module (MMEnc) aligns the vision and text modality knowledge into one unified item's multimodal representation; The aggregation module $Aggregator$ aggregates the neighbors' information with the help of the interacted graph $\mathcal{G}$; The fusion module $Fuser$ fuses multimodal representations and ID-based representations for top-K recommendation. The input and output of these modules are defined in Eq~\eqref{eq:mmrec},~\eqref{eq:aggregation},~\eqref{eq:fusion}. Next, we introduce their detailed structures.

\subsubsection{Multimodal Encoder Module}
In this module, we adopt the most advanced BEiT3~\cite{wang2022image} as the encoder backbone, with raw image and text as input. The MMEnc will align vision and text information via cross-modality experts~\cite{bao2022vlmo} and cross-attention based transformers. We train this module through the mask-then-predict strategy as shown in Eq~\eqref{eq:mmrec-loss} to ensure that the model have a better understanding of both vision and text modalities.

\subsubsection{Aggregation Module}
Following~\cite{zhou2023bootstrap,yu2023multi}, we use LightGCN~\cite{he2020lightgcn} to aggregate users and items representations from their neighbors. First of all, we adopt an embedding layer to users and items to get their embeddings $\mathbf{e}^i_{id},\mathbf{e}^u_{id}$. Stacking embeddings of all users and items together, we get the overall matrix $\mathbf{E}_{id}$. Then we can apply the LightGCN with $L$ layers defined in Sec.2 to aggregate neighbors ID-based information, and obtain $\mathbf{H}_{id}$, which is the representation matrix stacked by $\mathbf{h}^u_{id}$ and $\mathbf{h}^i_{id}$:
\begin{equation}
\begin{aligned}
    \mathbf{H}^{l+1}_{id} &= \hat{\mathbf{A}}\mathbf{H}^l_{id}, \quad \mathbf{H}^0_{id}=\mathbf{E}_{id},\quad l\in \{0,\ldots, L-1\}\,;\\
    \mathbf{H}_{id}&=\frac{1}{L+1}(\mathbf{H}^0+\mathbf{H}^1+\ldots+\mathbf{H}^L)\,.
    % \mathbf{H}_{id}&=\text{READOUT}(\mathbf{H}^0,\mathbf{H}^1,\ldots,\mathbf{H}^L)\,,
\end{aligned}
\end{equation}
% where $\text{READOUT}$ function can be any differentiable function, and we use the default mean function of LightGCN. $\mathbf{H}_{id}$ is the representation matrix stacked by $\mathbf{h}^u_{id}$ and $\mathbf{h}^i_{id}$.

Secondly, we build the item-side multimodal hidden representation $\mathbf{h}^i_{mm}$ as shown in Eq~\eqref{eq:item-mm}, where $\odot$ is the element-wise product, $\sigma$ is the sigmoid activation function, $MLP$ is the multi-layer perceptron. We 
adopt an adaptation layer of the encoded multimodal representation $\mathbf{h}^i_{enc}$ to roughly fuse the ID-based and modality-based knowledge, and get the content embedding $\mathbf{h}^i_{con}$ for each item $i$. Then we aggregate multimodal neighbors' information with a similarity matrix $\mathbf{S}$ into $\mathbf{h}^i_{mm}$. The matrix $\mathbf{S}$ is constructed by calculating items' multimodal information ($\mathbf{h}^i_{enc}$) similarity of each pair, and only preserve $K'$ most similarity edges (we set $K'=10$ following~\cite{yu2023multi}).
\begin{equation}\label{eq:item-mm}
\begin{aligned}
        \mathbf{h}^i_{con}&=\mathbf{e}^i_{id}\odot \sigma \left(MLP(\mathbf{h}^i_{enc})\right)\,,\\
    \mathbf{h}^i_{mm}&=\sum_{j\in \mathcal{I}}\mathbf{S}_{ij}\mathbf{h}^i_{con}\,.
\end{aligned}
\end{equation}

Finally, we build the user-side multimodal hidden representation $\mathbf{h}^u_{mm}$. Denote $\hat{\mathbf{R}}\in \mathbb{R}^{|\mathcal{U}|\times|\mathcal{I}|}$ as the normalized user-item interacted matrix (derived from top-right corner of $\hat{\mathbf{A}}$), then the aggregation process of user-side multimodal representation can be written as:
\begin{align}
    \mathbf{h}^u_{mm}&=\sum_{j\in \mathcal{I}}\hat{\mathbf{R}}_{uj}\mathbf{h}^j_{mm}\,.
\end{align}

\subsubsection{Fusion Module}
In the fusion module $Fuser$, we utilize the element-wise addition operation as presented in Eq~\eqref{eq:fm-implement} to fuse the multimodal and ID-based representation, and finally get a general representation for each item and user. They will be used for recommendation. This module can also be replaced by more complicated fusion operations like MLP or attention in current methods.
\begin{align}\label{eq:fm-implement}
    \mathbf{h}^i=\mathbf{h}^i_{mm}+\mathbf{h}^i_{id},\quad 
    \mathbf{h}^u=\mathbf{h}^u_{mm}+\mathbf{h}^u_{id}\,.
\end{align}

\subsection{Top-K Recommendation}
In the training stage, we use the common BPR loss defined in Eq.~\eqref{defi:bpr} to optimize the recommendation goal, with inner product as the score function and $i'$ as the negative sampled item:
\begin{align}\label{eq:bpr-loss}
    \mathcal{L}_{BPR}=\ln \sigma\left[ \mathbf{h}^i(\mathbf{h}^u)^{\intercal}-\mathbf{h}^{i'}(\mathbf{h}^u)^{\intercal}\right]\,.
\end{align}

In the recommendation stage, we calculate and rank the score of all user-item pairs given a user $u$: $s(u,i)=\mathbf{h}^i(\mathbf{h}^u)^{\intercal}$. Then, we choose $K$ top-ranked items as recommended items to the user.

\section{Training and Evaluating Align4Rec}\label{sec:train}
In this section, we will first introduce the training strategies proposed in Align4Rec, and then show the intermediate evaluation part to validate the effectiveness of multimodal information towards recommendation.

\subsection{Training Strategies}
In Align4Rec, we have three alignment losses (Eq.~\eqref{eq:mmrec-loss},~\eqref{eq:agg-loss},~\eqref{eq:ui-loss}) together with the recommendation BPR loss (Eq.~\eqref{eq:bpr-loss}) and regularization loss (Eq.~\eqref{eq:sim-loss}) to be optimized. However, optimizing them together with an end-to-end training strategy will encounter several problems. 

The first problem is convergence difficulty. As illustrated above, the inter-modality alignment requires our model to learn a unified multimodal representation that integrating the information in raw images and text, which requires a large amount of image-text pair data and more training time~\cite{radford2021learning}. On contrary, the recommendation-related tasks (modality-ID alignment and user-item alignment) usually converge quickly~\cite{zhang2022towards}. Therefore, training them end-to-end naively will make the recommendation-related tasks converge before the IMA task learns well, which indicates that the recommendation-related tasks cannot obtain the proper multimodal information. The second problem is joint-optimization difficulty. The multimodal encoder in the inter-modality alignment is composed of complicated transformers, while the recommendation-related tasks consist of simple fully-connected layers and graph aggregation layers. As a result, jointly training them together makes it hard for the optimization of the whole network structure.

Considering the difficulties above, in Align4Rec, we propose to separate and decouple the whole training process into two part: First, pre-training the inter-modality alignment task (named \textit{Pre-training}); Then, training the remaining two alignment tasks together with the recommendation goal (named \textit{Rec-training}) with weight hyper-parameters $\alpha$, $\beta$, and $\lambda$:
\begin{equation}\label{eq:train}
\begin{aligned}
    \textit{Pre-training: }&\max \mathcal{L}_{IMA}\,,\\
    \textit{Rec-training: }&\max \mathcal{L}_{BPR}+\alpha \mathcal{L}_{MIA}+\beta \mathcal{L}_{UIA}+\lambda \mathcal{L}_{reg}\,.
\end{aligned}
\end{equation}

\subsection{Intermediate Evaluation Protocols}
After separating the training process into two sub-processes, it is important to evaluate whether our multimodal encoder can generate features that are suitable and helpful for the recommendation task based on inter-modality alignment.
Previous methods just try to practically train models with multimodal features to validate their effectiveness, suffering from high training cost and long feedback latency. Therefore, we propose a set of intermediate evaluation protocols for multimodal recommendation in Align4Rec to \textbf{directly} evaluate the quality of multimodal features without any ID-based feature. In the following paragraphs, we suppose $\mathbf{h}^i_{mm}$ as item $i$'s multimodal feature.

\paragraph{Zero-Shot Recommendation} It evaluates whether multimodal features can correctly reflect user's interests based on historical interacted items, with three steps:
\begin{itemize}
    \item \textbf{Step I}. Construct user $u$'s interacted items list in time order. Select the most recent interacted item $i$ as the target item, the remaining items as the historical behavior $H_u$.
    \item \textbf{Step II}. Calculate the multimodal feature of user $u$ based on his/her history: $\mathbf{h}^u_{mm}=\frac{1}{|H_u|}\sum_{j\in H_u}\mathbf{h}^j_{mm}$.
    \item \textbf{Step III}. Calculated the similarity between $\mathbf{h}^u_{mm}$ and each item's multimodal feature in candidate set, and observe whether the target item $i$ can be recalled to $u$ based on top-K similar items.
\end{itemize}
In this protocol, $Recall$ will be larger if the similarity between $\mathbf{h}^{i}_{mm}$ and $\mathbf{h}^u_{mm}$ is large, \ie, historical items' multimodal feature of user $u$ is close to the target item's multimodal feature, with proper reflection on user's interests.

\paragraph{Item-CF Recommendation} It evaluates whether we can correctly recommend items with the CF method via only multimodal features, similar to item-CF~\cite{10.1145/371920.372071}.
\begin{itemize}
    \item \textbf{Step I}. Calculate item-CF score on each of two items according to~\cite{10.1145/371920.372071}.
    \item \textbf{Step II}. For each item $j$, select the item with the highest item-CF score as its target item $i$.
    \item \textbf{Step III}. Calculate the similarity between multimodal features of item $j$ and each item in candidate set, and observe whether $i$ can be recalled on top-K similar items.
\end{itemize}
In this protocol, if the similarity between items' multimodal features is in proportion to the item-CF score, the target item $i$ can be easier to be recalled, indicating multimodal features can properly represent items information.

\paragraph{Mask Modality Recommendation} It measures the difference in performance when we mask items' vision or text modality with a certain percentage. To be specific, we randomly mask $x\%$ of vision of text raw features and generate single-modality representations using $MMEec$. Then we repeat the steps in the above two protocols for recommendation.
